Untangling Dense Knots by Learning Task-Relevant Keypoints

Untangling ropes, wires, and cables is a challenging task for robots due to the high-dimensional configuration space, visual homogeneity, self-occlusions, and complex dynamics. We consider dense (tight) knots that lack space between self-intersections and present an iterative approach that uses learned geometric structure in configurations. We instantiate this into an algorithm, HULK: Hierarchical Untangling from Learned Keypoints, which combines learning-based perception with a geometric planner into a policy that guides a bilateral robot to untangle knots. To evaluate the policy, we perform experiments both in a novel simulation environment modelling cables with varied knot types and textures and in a physical system using the da Vinci surgical robot. We find that HULK is able to untangle cables with dense figure-eight and overhand knots and generalize to varied textures and appearances. We compare two variants of HULK to three baselines and observe that HULK achieves 43.3% higher success rates on a physical system compared to the next best baseline. HULK successfully untangles a cable from a dense initial configuration containing up to two overhand and figure-eight knots in 97.9% of 378 simulation experiments with an average of 12.1 actions per trial. In physical experiments, HULK achieves 61.7% untangling success, averaging 8.48 actions per trial. Supplementary material, code, and videos can be found at https://tinyurl.com/y3a88ycu.

==> 9-covid_one_pager.tex <==
\newpage
\appendix
\begin{LARGE}
\begin{center}
\textbf{Learning Robot Policies for Untangling Dense Knots in Linear Deformable Structures \\ Considerations for the Pandemic}
\end{center}
\end{LARGE}
\maketitle

It was not possible to perform physical evaluation of HULK during
COVID-19.  Initial results with real images suggest that the perception of
bounding boxes around knots and the contained pin /  pull points have
potential to be learned (Appendix \ref{sec:sim2real_details}).  We will perform extensive physical experiments
with varying materials and conditions using our ABB YuMi robot as soon as
possible and report results in the final version if accepted.

% The ongoing COVID-19 pandemic resulted in lab closures that prevented the authors from safely performing physical experiments at the time of submission. However, HULK was developed in a simulation environment built in Blender 2.8 similar to that of~\citet{sundaresan2020learning, ganapathi2020learning, seita2019deep, hoque2020visuospatial}. These works employed domain randomization to transfer deformable manipulation policies learned in simulation to the real world. We adopt many of the same domain randomization techniques from these works including variation over lighting intensity, camera position/orientation, and colors, textures, dimensions, and material properties for both simulated LDOs and the background manipulation surface. We present initial results for sim-to-real transfer of HULK's learned perception pipeline to RGB images of a real nylon rope in Appendix \ref{sec:sim2real_details}. The results demonstrate qualitative success with transferring predicted knot-bounding boxes and task-relevant keypoints, learned entirely in simulation, to real images of an LDO. 

% Besides transferring HULK's learned perception module to the real world, implementing the required manipulation primitives with a physical robot is the remaining next step. When we are able to gain access to the robotics lab, we plan to implement HULK on an ABB YuMi robot with dual grippers for bilateral manipulation support as in the work of ~\citet{lui2013tangled}. In Appendix \ref{sec:sim2real_details}, we include two grippers of the ABB YuMi robot in our LDO simulator to model the robot's motion trajectories and perform collision-checking. Additionally, experiments will be conducted with a nylon rope with physical properties visually similar to that of the simulated LDO, suggesting the manipulation actions of the grippers in the simulator will also be sufficient for untangling the real nylon rope. 

% We look forward to applying HULK to untangle real ropes, chords, and other LDOs once it can be done safely and will report .

